FLEdge: Benchmarking Federated Machine Learning Applications in Edge Computing Systems

Federated Learning (FL) has become a viable technique for realizing privacy-enhancing distributed deep learning on the network edge. Heterogeneous hardware, unreliable client devices, and energy constraints often characterize edge computing systems. In this paper, we propose FLEdge, which complements existing FL benchmarks by enabling a systematic evaluation of client capabilities. We focus on computational and communication bottlenecks, client behavior, and data security implications. Our experiments with models varying from 14K to 80M trainable parameters are carried out on dedicated hardware with emulated network characteristics and client behavior. We find that state-of-the-art embedded hardware has significant memory bottlenecks, leading to 4x longer processing times than on modern data center GPUs.

==> chapters/tables/02_fl_system_background.tex <==
With our hardware-centric benchmark, we build the bridge between essential functional components in FL systems and local training environments, energy efficiency, privacy, and client reliability to showcase their impact on overall FL system performance.

\subsection{Motivation for FL at the edge}
The vast majority of data is generated 



\subsection{Challenges of FL at the edge}








We start by going from the individual FL client, where training happens, to the server and associated FL aggregation strategies. The process for a single FL round is depicted in~\Cref{fig:system-design} and follows the design proposed by Bonawitz~et~al.~\cite{bonawitz2019}.

\subsection{Training}
Training an FL workload in an edge computing system is often subject to heterogeneous training performance in terms of computational speed and model quality (e.g., accuracy for classification tasks).

Heterogeneity in computational speed can originate from a variety of causes. 
The most prevailing is hardware heterogeneity, either due to long product life cycles in industrial systems controlled or due to a lack of infrastructure control.
For instance, widely used embedded devices for industrial edge require extensive reliability testing and, therefore, include hardware as old as five years \cite{siemens_edge}. 

At the same time, the model quality of FL workloads has received significant attention with two main streams of research: centralized and personalized FL. While centralized FL aims to create one global model for all clients, personalized FL has the objective to fit a model to clients individually and only incorporate global insights to a limited degree. For both disciplines, the computational loads on the clients are essentially identical \cite{chen2022}.

In recent research, the generational differences of devices within an FL system are usually neglected \cite{Wang2022_heterogen}, leaving open a key question for practitioners as to what devices to consider for FL workloads at all. In high-performance computing (HPC) research, micro-benchmarks for clients or hosts are an established method to identify performance bottlenecks, differences between system components, and their effects on the overall system performance \cite{mattson2020, awan2020}.

In contrast to HPC, where extensive client monitoring is widely applied, we only have very limited access to clients in FL systems and, therefore, require easily accessible and fast-to-interpret metrics. Since modern embedded devices are designed as system-on-a-chip (SoC), measuring their overall power consumption is trivial\footnote{Power measurements in virtualized cloud environments can only be approximated when knowing the underlying hardware \cite{Fieni2021}}. Paired with the training speed, i.e., the number of samples per second processed (SPS), we can derive the energy efficiency (\cref{eq:energy_efficiency}) of an embedded device for a given FL workload and optimize system hyper-parameters for optimal energy consumption.

\begin{equation} 
    \label{eq:energy_efficiency}
    \eta_e = \frac{\mathrm{SPS}}{W}
\end{equation}


\subsection{Communication}
The communication in edge computing systems between the embedded devices and the server depends on the environment. For industrial applications, communication can either be facilitated through a wired connection or via wireless technologies. While wired connections provide high stability and bandwidths, wireless technologies, such as 5G, LTE, or industrial WiFi, have a much more limited bandwidth.

As such, whenever communication increases, we have less time to spend on computation and become less efficient in terms of learning. Therefore, it is key to look into the share between computation and communication. We leverage Granularity (\cref{eq:granularity}) to express the ratio of computation and communication to determine the additional benefits of adding a certain device type to our FL system.

\begin{equation} 
    \label{eq:granularity}
    G = \frac{T_{\mathrm{Computation}}}{T_{\mathrm{Communication}}}
\end{equation}


\subsection{Privacy}
The importance of privacy varies by FL workload and the sensitivity of data. In FL systems, privacy is typically achieved by user-level differential privacy (DP). This is a method for applying Gaussian noise to client models before aggregation so that the likelihood of data leakage is close to 0. Precisely, DP is defined as $(\epsilon, \delta)-DP$, where $\epsilon$ defines the privacy budget and $\delta$ the data leakage probability. For FL workloads, we use $\epsilon$ to estimate the amount of information that has been processed through model aggregation. $\delta$ is typically set to the inverse of the total number of data points in the FL system, i.e., $\frac{1}{N}$. The noise we add to the models has a significant effect on the model quality.

To make FL workloads differentially private, we can use existing FL aggregation methods and add user-level DP on top of it (\cref{eq:userlevel-dp}, user-level DP with FedAvg, details in \Cref{sec:model-agg}). For user-level DP $z$ is the noise multiplier that controls the Gaussian noise $\mathcal{N}$ added to the model. $\mathcal{N}$ is defined with a mean of 0 and a standard deviation of $I\sigma^2_\Delta$, which ultimately depends on the number of clients we use in a single training round.

\begin{equation} 
    \label{eq:userlevel-dp}
    w^{t+1} = \frac{1}{M}(\sum_{m \in M} w_m^t + z * \mathcal{N}(0, I\sigma_{\Delta}^2))
\end{equation}

\subsection{Client Selection}
Client selection in FL systems happens randomly for a wide range of applications~\cite{mcmahan2017, li_fedprox2018, Reddi2020}. Yet, a typically neglected fact is the reliability of clients and their direct effect on model quality, privacy guarantees, and overall system efficiency.
In edge computing systems, typically, there is no dependency of the server on the clients \cite{}. Yet, for FL workloads, the server requires data from clients and, therefore, a timely and stable training process. In \Cref{eq:userlevel-dp}, $m$ defines a constant number of clients participating in a training round, while in reality, clients may drop out anytime. It is possible to select a replacement client, but this comes at the cost of additional block time for an FL training round to complete. The alternative is to aggregate all model updates that were received by the server. In case we are using DP, this requires us to re-adjust $I^2_\Delta$ for fewer clients and introduce more noise in order to provide the same privacy guarantees.


\subsection{Model aggregation \& validation}
\label{sec:model-agg}
Similar to hyperparameter optimization in deep learning, the core of FL workloads is the method for aggregating client models. There is a wide variety of aggregators that each address an individual problem of FL systems. The 


\subsection{Deep Learning Workload Coordination}

==> chapters/tables/granularity-table-main.tex <==
\begin{table}[!ht]
\caption{Granularity $G$ calculation to quantify the utility of deploying FL workloads based on compute vs. communication. OOM (= Out Of Memory) indicates the device is not capable of running a workload.}
\label{tab:granularity-network}
\scalebox{0.68}{
    \begin{tabular}{@{}ll|rrr|rrr@{}}
        \toprule
        & \multicolumn{1}{c}{} & \multicolumn{3}{c}{4G LTE}& \multicolumn{3}{c}{1 Gbit/s fiber} \\
        \midrule
        Dataset & Model & \multicolumn{1}{c}{RPi 4} & \multicolumn{1}{c}{Nano} & Orin & \multicolumn{1}{c}{RPi 4} & \multicolumn{1}{c}{Nano} & Orin\\ \midrule
        FEMNIST & CNN & 791 & 438& 579& 35000 & 19375& 25625 \\
        BLOND & CNN & 918 & 325& 155& 40625 & 14375& 6875\\
        BLOND & LSTM& 565 & 148& 92 & 25000 & 6563 & 4063\\
        BLOND & ResNet& 2076& 127& 53 & 91875 & 5625 & 2344\\
        BLOND & DenseNet& 828 & 51 & 23 & 36625 & 2250 & 1000\\
        Shakespeare & LSTM& 433 & 26 & 8& 19160 & 1152 & 371 \\
        Samsum& FLAN-T5 Small & OOM & OOM & 1.5& OOM & OOM & 65.7\\ 
        \bottomrule
        \bottomrule
    \end{tabular}
    }
\end{table}

==> chapters/tables/profiling_results.tex <==
\begin{tabular}{@{}llrr@{}}
    \toprule
    \textbf{Bottleneck}      & \textbf{Item}                        & \textbf{Orin} & \textbf{GPU} \\ \midrule
    \multirow{3}{*}{Compute} & Nb. of GPU SMs                       & 16            & 84           \\
                             & Compute Load per GPU SM              & 1200          & 170          \\
                             & CrossAttention Time (on GPU)         & 100ms         & 1.5ms        \\ \midrule
    \multirow{3}{*}{Memory}  & $\mathrm{Memory Bandwidth}^\ast$               & 175 GB/s      & 684 GB/s     \\
                             & CPU $\longrightarrow$ GPU Copy Operation & $20.8\mu\mathrm{s}$        & $8.9\mu\mathrm{s}$        \\
                             & CPU Memory Read Operation                   & $6\mu\mathrm{s}$           & $3\mu\mathrm{s}$          \\ \bottomrule
\end{tabular}

==> chapters/tables/speedup_table.tex <==
\begin{table}
    \centering
    \caption{Speedup comparison across device types, datasets, and ML models.}
    \label{tab:speedup-comparison}
    \scalebox{0.52}{
    \begin{adjustbox}{angle=90}
    \begin{tabular}{lll|rrrrr|rrrrr|rrrrr|rrrrr|rrrrr|rrrrr}
        \toprule
          &  & Step & \multicolumn{5}{c}{Batch Load} & \multicolumn{5}{c}{Forward} & \multicolumn{5}{c}{Loss Calc.} & \multicolumn{5}{c}{Backward} & \multicolumn{5}{c}{Optim. Step} & \multicolumn{5}{c}{Total} \\
         Dataset & Model  & Device & GPU & VM & Orin & Nano & RPi & GPU & VM & Orin & Nano & RPi & GPU & VM & Orin & Nano & RPi & GPU & VM & Orin & Nano & RPi & GPU & VM & Orin & Nano & RPi & GPU & VM & Orin & Nano & RPi \\
        \midrule
        \multirow[t]{20}{*}{BLOND} & \multirow[t]{5}{*}{CNN} & GPU & 1.0 & 1.17 & 2.12 & 1.72 & 1.51 & 1.0 & 32.87 & 1.54 & 37.49 & 238.08 & 1.0 & 1.44 & 2.27 & 34.84 & 2.82 & 1.0 & 32.19 & 1.79 & 12.92 & 87.14 & 1.0 & 14.54 & 3.05 & 23.01 & 65.84 & 1.0 & 3.52 & 2.18 & 4.48 & 12.88 \\
         &  & VM & 0.86 & 1.0 & 1.81 & 1.47 & 1.29 & 0.03 & 1.0 & 0.05 & 1.14 & 7.24 & 0.69 & 1.0 & 1.57 & 24.2 & 1.96 & 0.03 & 1.0 & 0.06 & 0.4 & 2.71 & 0.07 & 1.0 & 0.21 & 1.58 & 4.53 & 0.28 & 1.0 & 0.62 & 1.27 & 3.66 \\
         &  & Orin & 0.47 & 0.55 & 1.0 & 0.81 & 0.71 & 0.65 & 21.28 & 1.0 & 24.28 & 154.16 & 0.44 & 0.64 & 1.0 & 15.37 & 1.24 & 0.56 & 17.97 & 1.0 & 7.21 & 48.64 & 0.33 & 4.77 & 1.0 & 7.55 & 21.61 & 0.46 & 1.61 & 1.0 & 2.05 & 5.9 \\
         &  & Nano & 0.58 & 0.68 & 1.23 & 1.0 & 0.88 & 0.03 & 0.88 & 0.04 & 1.0 & 6.35 & 0.03 & 0.04 & 0.07 & 1.0 & 0.08 & 0.08 & 2.49 & 0.14 & 1.0 & 6.75 & 0.04 & 0.63 & 0.13 & 1.0 & 2.86 & 0.22 & 0.79 & 0.49 & 1.0 & 2.88 \\
         &  & RPi & 0.66 & 0.77 & 1.4 & 1.14 & 1.0 & 0.0 & 0.14 & 0.01 & 0.16 & 1.0 & 0.36 & 0.51 & 0.8 & 12.37 & 1.0 & 0.01 & 0.37 & 0.02 & 0.15 & 1.0 & 0.02 & 0.22 & 0.05 & 0.35 & 1.0 & 0.08 & 0.27 & 0.17 & 0.35 & 1.0 \\ \cmidrule{2-33}
         & \multirow[t]{5}{*}{LSTM} & GPU & 1.0 & 0.12 & 2.79 & 1.32 & 0.27 & 1.0 & 176.84 & 1.59 & 26.07 & 199.37 & 1.0 & 1.25 & 2.12 & 38.2 & 2.45 & 1.0 & 135.6 & 1.46 & 15.27 & 105.67 & 1.0 & 74.81 & 3.46 & 17.74 & 70.91 & 1.0 & 16.75 & 2.8 & 4.2 & 15.92 \\
         &  & VM & 8.17 & 1.0 & 22.82 & 10.75 & 2.2 & 0.01 & 1.0 & 0.01 & 0.15 & 1.13 & 0.8 & 1.0 & 1.7 & 30.54 & 1.96 & 0.01 & 1.0 & 0.01 & 0.11 & 0.78 & 0.01 & 1.0 & 0.05 & 0.24 & 0.95 & 0.06 & 1.0 & 0.17 & 0.25 & 0.95 \\
         &  & Orin & 0.36 & 0.04 & 1.0 & 0.47 & 0.1 & 0.63 & 110.94 & 1.0 & 16.36 & 125.07 & 0.47 & 0.59 & 1.0 & 17.99 & 1.15 & 0.69 & 92.96 & 1.0 & 10.47 & 72.44 & 0.29 & 21.6 & 1.0 & 5.12 & 20.47 & 0.36 & 5.99 & 1.0 & 1.5 & 5.69 \\
         &  & Nano & 0.76 & 0.09 & 2.12 & 1.0 & 0.2 & 0.04 & 6.78 & 0.06 & 1.0 & 7.65 & 0.03 & 0.03 & 0.06 & 1.0 & 0.06 & 0.07 & 8.88 & 0.1 & 1.0 & 6.92 & 0.06 & 4.22 & 0.2 & 1.0 & 4.0 & 0.24 & 3.98 & 0.67 & 1.0 & 3.79 \\
         &  & RPi & 3.72 & 0.46 & 10.38 & 4.89 & 1.0 & 0.01 & 0.89 & 0.01 & 0.13 & 1.0 & 0.41 & 0.51 & 0.87 & 15.58 & 1.0 & 0.01 & 1.28 & 0.01 & 0.14 & 1.0 & 0.01 & 1.06 & 0.05 & 0.25 & 1.0 & 0.06 & 1.05 & 0.18 & 0.26 & 1.0 \\ \cmidrule{2-33}
         & \multirow[t]{5}{*}{ResNet} & GPU & 1.0 & 0.14 & 2.68 & 0.9 & 0.27 & 1.0 & 64.84 & 1.59 & 6.01 & 628.17 & 1.0 & 3.43 & 2.16 & 12.79 & 2.32 & 1.0 & 128.97 & 2.04 & 5.76 & 115.22 & 1.0 & 74.94 & 3.04 & 21.12 & 225.22 & 1.0 & 34.44 & 2.63 & 6.42 & 104.54 \\
         &  & VM & 7.32 & 1.0 & 19.59 & 6.57 & 1.99 & 0.02 & 1.0 & 0.02 & 0.09 & 9.69 & 0.29 & 1.0 & 0.63 & 3.73 & 0.68 & 0.01 & 1.0 & 0.02 & 0.04 & 0.89 & 0.01 & 1.0 & 0.04 & 0.28 & 3.01 & 0.03 & 1.0 & 0.08 & 0.19 & 3.04 \\
         &  & Orin & 0.37 & 0.05 & 1.0 & 0.34 & 0.1 & 0.63 & 40.71 & 1.0 & 3.77 & 394.37 & 0.46 & 1.58 & 1.0 & 5.91 & 1.07 & 0.49 & 63.21 & 1.0 & 2.82 & 56.47 & 0.33 & 24.68 & 1.0 & 6.95 & 74.17 & 0.38 & 13.11 & 1.0 & 2.44 & 39.8 \\
         &  & Nano & 1.11 & 0.15 & 2.98 & 1.0 & 0.3 & 0.17 & 10.79 & 0.26 & 1.0 & 104.5 & 0.08 & 0.27 & 0.17 & 1.0 & 0.18 & 0.17 & 22.4 & 0.35 & 1.0 & 20.01 & 0.05 & 3.55 & 0.14 & 1.0 & 10.67 & 0.16 & 5.37 & 0.41 & 1.0 & 16.29 \\
         &  & RPi & 3.67 & 0.5 & 9.83 & 3.3 & 1.0 & 0.0 & 0.1 & 0.0 & 0.01 & 1.0 & 0.43 & 1.48 & 0.93 & 5.52 & 1.0 & 0.01 & 1.12 & 0.02 & 0.05 & 1.0 & 0.0 & 0.33 & 0.01 & 0.09 & 1.0 & 0.01 & 0.33 & 0.03 & 0.06 & 1.0 \\ \cmidrule{2-33}
         & \multirow[t]{5}{*}{DenseNet} & GPU & 1.0 & 0.18 & 3.32 & 1.57 & 0.35 & 1.0 & 55.21 & 2.0 & 6.77 & 468.94 & 1.0 & 2.7 & 2.66 & 5.26 & 3.05 & 1.0 & 60.02 & 1.91 & 5.86 & 82.31 & 1.0 & 44.62 & 2.59 & 13.51 & 174.34 & 1.0 & 26.57 & 2.79 & 6.2 & 104.55 \\
         &  & VM & 5.41 & 1.0 & 17.97 & 8.51 & 1.9 & 0.02 & 1.0 & 0.04 & 0.12 & 8.49 & 0.37 & 1.0 & 0.99 & 1.95 & 1.13 & 0.02 & 1.0 & 0.03 & 0.1 & 1.37 & 0.02 & 1.0 & 0.06 & 0.3 & 3.91 & 0.04 & 1.0 & 0.11 & 0.23 & 3.93 \\
         &  & Orin & 0.3 & 0.06 & 1.0 & 0.47 & 0.11 & 0.5 & 27.65 & 1.0 & 3.39 & 234.82 & 0.38 & 1.01 & 1.0 & 1.98 & 1.15 & 0.52 & 31.45 & 1.0 & 3.07 & 43.13 & 0.39 & 17.23 & 1.0 & 5.22 & 67.34 & 0.36 & 9.52 & 1.0 & 2.22 & 37.46 \\
         &  & Nano & 0.64 & 0.12 & 2.11 & 1.0 & 0.22 & 0.15 & 8.15 & 0.29 & 1.0 & 69.23 & 0.19 & 0.51 & 0.5 & 1.0 & 0.58 & 0.17 & 10.25 & 0.33 & 1.0 & 14.06 & 0.07 & 3.3 & 0.19 & 1.0 & 12.9 & 0.16 & 4.28 & 0.45 & 1.0 & 16.86 \\
         &  & RPi & 2.84 & 0.53 & 9.44 & 4.47 & 1.0 & 0.0 & 0.12 & 0.0 & 0.01 & 1.0 & 0.33 & 0.88 & 0.87 & 1.72 & 1.0 & 0.01 & 0.73 & 0.02 & 0.07 & 1.0 & 0.01 & 0.26 & 0.01 & 0.08 & 1.0 & 0.01 & 0.25 & 0.03 & 0.06 & 1.0 \\ \cmidrule{1-33}
        \multirow[t]{5}{*}{FEMNIST} & \multirow[t]{5}{*}{CNN} & GPU & 1.0 & 1.17 & 25.07 & 6.59 & 2.48 & 1.0 & 32.68 & 3.72 & 7.82 & 92.02 & 1.0 & 1.95 & 3.2 & 6.7 & 4.19 & 1.0 & 13.84 & 2.72 & 4.46 & 19.01 & 1.0 & 8.5 & 4.3 & 11.23 & 16.62 & 1.0 & 7.43 & 11.86 & 8.53 & 14.95 \\
         &  & VM & 0.86 & 1.0 & 21.52 & 5.66 & 2.12 & 0.03 & 1.0 & 0.11 & 0.24 & 2.82 & 0.51 & 1.0 & 1.64 & 3.44 & 2.15 & 0.07 & 1.0 & 0.2 & 0.32 & 1.37 & 0.12 & 1.0 & 0.51 & 1.32 & 1.96 & 0.13 & 1.0 & 1.6 & 1.15 & 2.01 \\
         &  & Orin & 0.04 & 0.05 & 1.0 & 0.26 & 0.1 & 0.27 & 8.78 & 1.0 & 2.1 & 24.73 & 0.31 & 0.61 & 1.0 & 2.1 & 1.31 & 0.37 & 5.09 & 1.0 & 1.64 & 7.0 & 0.23 & 1.98 & 1.0 & 2.61 & 3.86 & 0.08 & 0.63 & 1.0 & 0.72 & 1.26 \\
         &  & Nano & 0.15 & 0.18 & 3.8 & 1.0 & 0.38 & 0.13 & 4.18 & 0.48 & 1.0 & 11.78 & 0.15 & 0.29 & 0.48 & 1.0 & 0.62 & 0.22 & 3.1 & 0.61 & 1.0 & 4.26 & 0.09 & 0.76 & 0.38 & 1.0 & 1.48 & 0.12 & 0.87 & 1.39 & 1.0 & 1.75 \\
         &  & RPi & 0.4 & 0.47 & 10.13 & 2.66 & 1.0 & 0.01 & 0.36 & 0.04 & 0.08 & 1.0 & 0.24 & 0.46 & 0.76 & 1.6 & 1.0 & 0.05 & 0.73 & 0.14 & 0.23 & 1.0 & 0.06 & 0.51 & 0.26 & 0.68 & 1.0 & 0.07 & 0.5 & 0.79 & 0.57 & 1.0 \\ \cmidrule{1-33}
        \multirow[t]{5}{*}{Shakespeare} & \multirow[t]{5}{*}{LSTM} & GPU & 1.0 & 4.89 & 1.9 & 7.21 & 3.75 & 1.0 & 89.61 & 1.76 & 5.93 & 172.09 & 1.0 & 26.71 & 2.35 & 18.22 & 3.11 & 1.0 & 53.83 & 3.12 & 4.42 & 186.93 & 1.0 & 53.35 & 2.84 & 10.65 & 131.42 & 1.0 & 53.6 & 2.64 & 8.21 & 135.72 \\
         &  & VM & 0.2 & 1.0 & 0.39 & 1.47 & 0.77 & 0.01 & 1.0 & 0.02 & 0.07 & 1.92 & 0.04 & 1.0 & 0.09 & 0.68 & 0.12 & 0.02 & 1.0 & 0.06 & 0.08 & 3.47 & 0.02 & 1.0 & 0.05 & 0.2 & 2.46 & 0.02 & 1.0 & 0.05 & 0.15 & 2.53 \\
         &  & Orin & 0.53 & 2.57 & 1.0 & 3.79 & 1.97 & 0.57 & 50.92 & 1.0 & 3.37 & 97.78 & 0.43 & 11.39 & 1.0 & 7.77 & 1.33 & 0.32 & 17.26 & 1.0 & 1.42 & 59.93 & 0.35 & 18.81 & 1.0 & 3.76 & 46.34 & 0.38 & 20.34 & 1.0 & 3.12 & 51.5 \\
         &  & Nano & 0.14 & 0.68 & 0.26 & 1.0 & 0.52 & 0.17 & 15.12 & 0.3 & 1.0 & 29.03 & 0.05 & 1.47 & 0.13 & 1.0 & 0.17 & 0.23 & 12.17 & 0.71 & 1.0 & 42.27 & 0.09 & 5.01 & 0.27 & 1.0 & 12.34 & 0.12 & 6.53 & 0.32 & 1.0 & 16.53 \\
         &  & RPi & 0.27 & 1.31 & 0.51 & 1.92 & 1.0 & 0.01 & 0.52 & 0.01 & 0.03 & 1.0 & 0.32 & 8.6 & 0.75 & 5.86 & 1.0 & 0.01 & 0.29 & 0.02 & 0.02 & 1.0 & 0.01 & 0.41 & 0.02 & 0.08 & 1.0 & 0.01 & 0.39 & 0.02 & 0.06 & 1.0 \\
        \bottomrule \bottomrule
    \end{tabular}
    \end{adjustbox}
    }
\end{table}

==> chapters/tables/system_metrics.tex <==
\begin{wraptable}{c}[\dimexpr\columnwidth+\columnsep\relax]{13cm}
    \centering
    \caption{System metrics for our energy efficiency experiments. We report CPU, memory, and GPU utilization. Note: The Nanos do not have dedicated VRAM as they are an SoC. As such, we cannot report GPU memory statistics.}
    \label{tab:hw-stats-appendix}
    \scalebox{0.63}{
        \begin{adjustbox}{angle=0} 
            \begin{tabular}{lll|rrr|rr|rr|r}
            \toprule
             & & & \multicolumn{3}{c}{CPU Util. Avg. (\%)}& \multicolumn{2}{c}{Memory (MB)}   & \multicolumn{2}{c}{GPU} &  Power (W)        \\
            Dataset                    & Model                  & Device    & 01-min & 05-min   & 15-min    & Process   & Total         & Util. (\%)    & Memory (MB) & Total \\
            \midrule
            \multirow[t]{20}{*}{BLOND} & \multirow[t]{5}{*}{CNN} & GPU      & 4±3   & 3±1       & 2±1       & 589±2     & 4027±1720     & 1±0           & 1940±305& 61±5 \\
             &                                                   & VM       & 62±32 & 68±31     & 68±34     & 555±104   & 1664±784      & N/A           & N/A     & 50±0 \\
             &                                                   & Orin     & 36±12 & 30±8      & 39±12     & 465±2     & 4541±1472     & N/A           & N/A     & 12±5 \\
             &                                                   & Nano     & 73±20 & 69±19     & 69±22     & 884±222   & 1724±226      & N/A           & N/A     & 5±1 \\
             &                                                   & RPi      & 54±21 & 56±19     & 69±35     & 368±9     & 1156±350      & N/A           & N/A     & 6±1 \\
             \cmidrule{2-11}
             & \multirow[t]{5}{*}{DenseNet}                      & GPU      & 5±4   & 3±2       & 3±1       & 592±3     & 4014±1710     & 60±4          & 1960±400& 63±2\\
             &                                                   & VM       & 76±26 & 80±24     & 81±23     & 686±116   & 2421±914      & 50±0          & N/A     & 50±0 \\
             &                                                   & Orin     & 44±10 & 37±3      & 38±5      & 469±2     & 4862±1612     & 13±5          & N/A     & 12±5\\
             &                                                   & Nano     & 76±19 & 74±16     & 73±17     & 828±241   & 1740±204      & 5±1           & N/A     & 5±1 \\
             &                                                   & RPi      & 84±21 & 82±10     & 78±8      & 542±61    & 1514±307      & 7±1           & N/A     & 7±1 \\
             \cmidrule{2-11}
             & \multirow[t]{5}{*}{LSTM}                          & GPU      & 3±3   & 3±1       & 3±1       & 589±3     & 3972±1551     & 60±4          & 1950±70 & 66±3 \\
             &                                                   & VM       & 69±29 & 73±28     & 70±31     & 554±113   & 2074±866      & 50±0          & N/A     & 50±0 \\
             &                                                   & Orin     & 36±9  & 31±6      & 38±10     & 465±2     & 4440±1377     & 13±5          & N/A     & 11±4 \\
             &                                                   & Nano     & 72±19 & 69±17     & 72±18     & 800±236   & 1701±240      & 5±1           & N/A     & 5±1 \\
             &                                                   & RPi      & 45±13 & 51±9      & 68±25     & 388±22    & 1181±346      & 6±1           & N/A     & 6±1 \\
             \cmidrule{2-11}
             & \multirow[t]{5}{*}{ResNet}                        & GPU      & 3±2   & 3±1       & 3±1       & 591±2     & 3988±1721     & 61±1          & 1959±203& 66±4 \\
             &                                                   & VM       & 70±27 & 77±27     & 77±27     & 709±122   & 2218±875      & 50±0          & N/A     & 50±0 \\
             &                                                   & Orin     & 40±10 & 34±2      & 38±8      & 470±2     & 4847±1602     & 13±5          & N/A     & 13±5 \\
             &                                                   & Nano     & 75±21 & 73±18     & 72±17     & 846±225   & 1741±208      & 5±2           & N/A     & 5±2 \\
             &                                                   & RPi      & 83±24 & 70±15     & 73±15     & 577±76    & 1548±317      & 7±1           & N/A     & 7±1 \\
             \cmidrule{1-11}
            \multirow[t]{5}{*}{FEMNIST} & \multirow[t]{5}{*}{CNN}& GPU      & 5±1   & 4±1       & 3±1       & 681±8     & 5887±1186     & 75±6          & 1920±311& 73±12 \\
             &                                                   & VM       & 96±12 & 95±12     & 92±14     & 544±301   & 2428±694      & 50±0          & N/A     & 50±0 \\
             &                                                   & Orin     & 28±9  & 34±9      & 45±15     & 690±9     & 6532±1202     & 11±2          & N/A     & 10±6 \\
             &                                                   & Nano     & 93±14 & 93±13     & 92±13     & 645±140   & 1672±93       & 6±1           & N/A     & 6±1 \\
             &                                                   & RPi      & 98±11 & 98±7      & 97±7      & 674±85    & 1974±354      & 6±1           & N/A     & 6±1 \\
             \cmidrule{1-11}
            \multirow[t]{5}{*}{Shakespeare} & \multirow[t]{5}{*}{LSTM}& GPU & 3±1   & 3±0       & 3±0       & 454±1     & 7375±907      & 93±5          & 2300±190& 94±8 \\
             &                                                   & VM       & 85±18 & 85±17     & 86±17     & 2026±415  & 3914±216      & 50±0          & N/A     & 50±0 \\
             &                                                   & Orin     & 34±9  & 35±2      & 37±5      & 462±4     & 4092±1312     & 17±11         & N/A     & 28±4 \\
             &                                                   & Nano     & 63±22 & 70±20     & 84±13     & 740±232   & 1731±207      & 5±2           & N/A     & 5±2 \\
             &                                                   & RPi      & 77±17 & 92±5      & 100±0     & 424±22    & 1411±249      & 7±1           & N/A     & 7±1 \\
            \cmidrule{1-11}
            \multirow[t]{1}{*}{Samsum}&\multirow[t]{1}{*}{FLAN-T5 (BS = 32)}& Orin  & 12±1 & 11±3 & 11±1    & 1105±17   & 18931±247     & 74±2          & 18931±247 & 41±4 \\ 
             
            \bottomrule \bottomrule
            \end{tabular}
        \end{adjustbox}
    }
\end{wraptable}


==> chapters/tables/t5-training.tex <==
\begin{tabular}{@{}llclrrrrrr@{}}
\toprule
& & \multicolumn{1}{l}{} & \multicolumn{6}{c}{Step time (in s)} & \multicolumn{1}{c}{$\eta_e$} \\ 
\multicolumn{1}{l|}{Device} & Dataset & \multicolumn{1}{l|}{Model} & \shortstack{Batch \\ Loading} & \multicolumn{1}{l}{Forw.} & \multicolumn{1}{l}{\shortstack{Loss \\ Calc.}} & \multicolumn{1}{l}{Backw.} & \multicolumn{1}{l}{Optim. Step} & \multicolumn{1}{l|}{Total} & \multicolumn{1}{l}{Total}                        \\ \midrule
\multicolumn{1}{l|}{\textbf{GPU}}             & \multirow{4}{*}{JFLEG} & \multicolumn{1}{c|}{\multirow{4}{*}{\shortstack{T5-small \\ (60M params)}}} & \multicolumn{1}{r}{\textbf{0.00}} & \textbf{0.02}                             & \textbf{N/A}                           & \textbf{0.35}                             & \textbf{0.62}                               & \multicolumn{1}{r|}{\textbf{0.99}}  & \textbf{0.36}                                             \\
\multicolumn{1}{l|}{\textbf{Orin (FP)}} &                        & \multicolumn{1}{c|}{}                                       & \multicolumn{1}{r}{\textbf{0.00}} & \textbf{0.04}                             & \textbf{N/A}                            & \textbf{1.79}                              & \textbf{3.12}                               & \multicolumn{1}{r|}{\textbf{4.95}}  & \textbf{0.24}                                             \\
\multicolumn{1}{l|}{Orin (30W)}  &                        & \multicolumn{1}{c|}{}                                       & \multicolumn{1}{r}{0.00} & 0.05                             & N/A                            & 3.59                              & 6.25                               & \multicolumn{1}{r|}{9.89}  & 0.22                                             \\
\multicolumn{1}{l|}{Orin (15W)}  &                        & \multicolumn{1}{c|}{}                                       & \multicolumn{1}{r}{0.00} & 0.08                             & N/A                            & 6.37                              & 11.11                              & \multicolumn{1}{r|}{17.56} & 0.19                                             \\
 \bottomrule
\end{tabular}
